Integrating High-Dimensional Functions Deterministically

We design a Quasi-Polynomial time deterministic approximation algorithm for computing the integral of a multi-dimensional separable function, supported by some underlying hyper-graph structure, appropriately defined. Equivalently, our integral is the partition function of a graphical model with continuous potentials. While randomized algorithms for high-dimensional integration are widely known, deterministic counterparts generally do not exist. We use the correlation decay method applied to the Riemann sum of the function to produce our algorithm. For our method to work, we require that the domain is bounded and the hyper-edge potentials are positive and bounded on the domain. We further assume that upper and lower bounds on the potentials separated by a multiplicative factor of $1 + O(1/\Delta^2)$, where $\Delta$ is the maximum degree of the graph. When $\Delta = 3$, our method works provided the upper and lower bounds are separated by a factor of at most $1.0479$. To the best of our knowledge, our algorithm is the first deterministic algorithm for high-dimensional integration of a continuous function, apart from the case of trivial product form distributions.

==> sections/algorithm.tex <==
This section will be dedicated to the algorithm used to approximate the value $Z(G)$. The primary piece in this algorithm, present in algorithm \ref{alg:prob}, will be a recursive algorithm to approximate the value of $x(G, v \la m,\beta)$.

\SetKwComment{Comment}{\# }{}
\begin{algorithm}[ht]
\caption{ApproxProb}\label{alg:prob}
\KwData{Hypergraph $G$,  Constraints $\beta$, Recursion Depth $d$, Assignment $y$}
\KwResult{Estimate $\tilde x(G, v \la m, \beta)$ of $x(G, v \la m, \beta)$}
\lIf{$d=0$}{\Return $\frac{1}{N}$}
Let $v_1, \ldots v_{\eta'}$ be the unconstrained neighbors of $v$\;\\
\For{$j \in [1,{\eta'}]$}{
\For{$y_1, \ldots y_j \in [0,N-1]$}{
Let $\tilde x(\bar y) = \operatorname{ApproxProb}(G \setminus v, (\beta, (v_i \la y_i, i < j)), d-1, y_j)$\;
}
}
\Return $g_m(\tilde \x)$ \Comment*[l]{where $g_m$ is defined in equation \ref{eq:g_m}}
\end{algorithm}
\begin{lemma}
\label{prob bound}
Algorithm \ref{alg:prob} will produce an estimate $\tilde x(G, v \la m, \beta)$ satisfying
\[|\tilde x(G, v \la m, \beta) - x(G, v \la m, \beta)| \leq (1 - \delta)^d.\]
This estimate will be computed in time $O(N^{\eta d})$.
\end{lemma}
\begin{proof}
We will prove the above theorem by induction. When $d=0$, the difference is trivially bounded by 1, so the theorem will hold. For $d > 1$, we have by induction that the coordinates of $\tilde \x$ computed in the highest level run of the algorithm differ from the coordinates of $\x$ by at most $(1-\delta)^{d-1}$. Further, by the mean value theorem, there must be some linear interpolation $\hat \x$ of $\tilde \x$ and $\x$ which satisfies
\[g_m(\tilde \x) - g_m(\x) = \nabla g_m(\hat \x) \cdot (\tilde \x - \x).\]
Thus, we can use theorem \ref{Bounded Gradients} to conclude that
\[|g_m(\tilde \x) - g_m(\x)| \leq \|\nabla g_m(\hat \x)\|_1 \|(\tilde \x - \x)\|_\infty \leq (1-\delta)^d.\]

Additionally, we wish to analyze the runtime of algorithm \ref{alg:prob}. We will let $T(d)$ denote the runtime of the algorithm with recursion depth $d$, and observe that $T(0) = O(1)$. For higher values of $d$, the limiting step will be the runtime of the recursive calls. There will be exactly $N^{\eta'}$ such calls, and each one will take at most $O({\eta'})$ time to update the value of $\beta$. Thus, we get that $T(d) = N^{\eta'} O({\eta'}) T(d-1)$, implying that $T(d) = O(N^{\eta d})$, since ${\eta'} \leq \eta$. 
\end{proof}


Before we analyze the full algorithm, we will make an observation about the function $g_m$. In particular, we will require the following Lemma, which we will prove in the appendix.

\begin{lemma}
\label{g_m lower lemma}
For any vector of marginal probabilities $\x$, we have
\[g_m(\x) \geq \frac{1}{\sqrt{2}N},\]
as long as the underlying hypergraph $G$ is connected.
\end{lemma}
At a high level, this proof follows from applying the potential function bounds in equation \ref{eq:Phi assum} to equation \ref{eq:g_m}. With this Lemma, we conclude with the following theorem.

\begin{algorithm}[ht]
\caption{ApproxZ}\label{alg:Z}
\KwData{Hypergraph $G$, Recursion Depth $d$}
\KwResult{Estimate $\tilde Z(G)$ of $Z(G)$}
Let $z\_inv \la 1$ and $\beta \la \{\}$\;\\
\For{$v \in V$}{
$z\_inv \la z\_inv * \rm ApproxProb(G, \beta, d, 0)$\;\\
$\beta \la (\beta, v \la 0)$\;
}
\Return $f(\0)/ z\_inv$
\end{algorithm}
\begin{theorem}
\label{final alg}
The estimate $\tilde Z(G)$ of $Z(G)$ produced by algorithm \ref{alg:Z} will satisfy
\[1 - O(1/n) \leq \frac{\tilde Z(G)}{Z(G)} \leq 1 + O(1/n)\]
for some $d = O(\log(Nn))$. This estimate will be computed in time $N^{O(\eta \log( N n))}$.
\end{theorem}
\begin{proof}
Order the vertices $v_1$ to $v_n$ in the same order they are iterated in algorithm \ref{alg:Z}, and let $\beta_i = (v_j \la 0, j \leq i)$ as in the end of section \ref{definitions}. Set $d = \log_{1 - \delta}(\frac{1}{\sqrt{2}Nn^2})$. This will result in our approximations $\tilde x(G, v_i \la 0, \beta_{i-1})$ computed in the algorithm to satisfy
\[| x(G, v_i \la 0, \beta_{i-1}) - \tilde x(G, v_i \la 0, \beta_{i-1})|
\leq (1 - \delta)^d = \frac{1}{\sqrt{2}Nn^2} \leq \frac{\tilde x(G, v_i \la 0, \beta_{i-1})}{n^2}\]
by Lemma \ref{prob bound} and \ref{g_m lower lemma}. Dividing both sides by $\tilde x(G, v_i \la 0, \beta_{i-1})$, we get
\[\bigg |  \frac{ x(G, v_i \la 0, \beta_{i-1})}{\tilde x(G, v_i \la 0, \beta_{i-1})} - 1 \bigg | \leq \frac{1}{n^2}.
\]
Next, notice that 
\[\frac{\tilde Z(G)}{Z(G)} = \frac{f(\0) \prod\limits_{i = 1}^{n} \tilde x^{-1}(G, v_i \la 0)}{f(\0) \prod\limits_{i = 1}^{n} x^{-1}(G, v_i \la 0)} = \frac{\prod\limits_{i = 1}^{n} x(G, v_i \la 0)}{\prod\limits_{i = 1}^{n} \tilde x(G, v_i \la 0)},\]
by equation \ref{eq:Z-unfurl}. Therefore, the estimate $\tilde Z$ produced by algorithm \ref{alg:Z} will satisfy
\[\(1- \frac{1}{n^2}\)^n = 1 - O(1/n) \leq \frac{\tilde Z(G)}{Z(G)} \leq 1 + O(1/n) \leq \(1 + \frac{1}{n^2}\)^n.\]
The runtime of this algorithm will be dominated by the calls to the function ApproxProb, which each take time $O(N^{\eta d})$ by Lemma \ref{prob bound}. Further, notice that $d = O(\log(Nn))$ since $(1 - \delta) < 1$. Thus, since there are $n$ calls to this function with this $d$, the algorithm will take time $N^{O(\eta \log( Nn))}$.
\end{proof}




==> sections/integrals.tex <==
In this section, we will present one method for relating the value of a Riemann sum to the value of the corresponding integral, based on bounding the functions $l2$-norm. This process will conclude with a short proof of theorem \ref{main result}. 

\begin{lemma}
\label{integral approx}
Suppose we have a function $f$ defined as in equation \ref{eq:f def}, where each function $\Phi_e$ is differentiable and satisfies $\|\nabla \Phi_e(\x)\|_2 \leq kc_e$ for every $\x \in [0,1]^n$. Then,
\[\( 1 - \frac{\sqrt{n}k}{N} \)^{|E|} 
\leq \frac{\int 1(\y \in [0,1]^n) f(\y) d\lambda}{Z(G)/N^n}
\leq \( 1 + \frac{\sqrt{n}k}{N} \)^{|E|}
,\]
where $Z(G)$ is defined as in equation \ref{eq:Z def}.
\end{lemma}

\begin{proof}
Pick any vector $\y \in \D$, and let $\y'$ be any vector satisfying $y_i \leq y_i' < y_i + 1/N$ for each index $i$. We will denote the set of all such $\y'$ as $\D_\y$. Notice that $\|\y - \y'\|_2 \leq \frac{\sqrt{n}}{N}$. Thus, for every edge $e \in E$, we have 
\[\Phi_e(\y) - \frac{\sqrt{n}}{N} k c_e \leq \Phi_e(\y') \leq \Phi_e(\y) + \frac{\sqrt{n}}{N}kc_e. \]
Using this, we see
\begin{align*}
\frac{\int_{\D_\y} f(\x) d\x}{f(\y)/N^n}
\leq \frac {\int_{\D_\y} \prod\limits_{e \in E} \(\Phi_e(\y) + \frac{\sqrt{n}}{N}kc_e d\x \)}{\prod\limits_{e \in E} \Phi_e(\y)/N^n}
= \frac{\prod\limits_{e \in E}\(\Phi_e(\y) + \frac{\sqrt{n}}{N}kc_e\)}{\prod\limits_{e\in E} \Phi_e(\y)}
\leq \(
1 + \frac{\sqrt{n}k}{N}
\)^{|E|},
\end{align*}
where the first inequality follows from the above equation, and the second inequality follows from the assumption in equation \ref{eq:Phi assum}. Similar reasoning will yield that 
$\frac{\int_{\D_\y} f(\x) d\x}{f(\y)/N^n} \geq \bigg (
1 - \frac{\sqrt{n}k}{N}
\bigg )^{|E|}$.
Finally, we observe that
\[\frac{\int 1(\y \in [0,1]^n) f(\y) d\lambda}{Z(G)/N^n} = \frac{\sum\limits_{\y \in \D} \int_{\D_\y} f(\x) d\x}{\sum\limits_{\y \in \D} f(\y)/N^n} \leq \max_{\y \in \D} \frac{\int_{\D_\y} f(\x) d\x}{f(\y)/N^n} \leq \(
1 + \frac{\sqrt{n}k}{N}
\)^{|E|},\]
with similar logic yielding
\[\frac{\int 1(\y \in [0,1]^n) f(\y) d\lambda}{Z(G)/N^n} \geq \( 1 - \frac{\sqrt{n}k}{N} \)^{|E|}.\]
\end{proof}
We are now ready to prove our main result.

\begin{proof} \textbf{of Theorem \ref{main result}}
Let $N = k n^{3/2} |E|$. By Lemma \ref{integral approx}, we will have that
\[e^{-1/n} \leq \frac{\int 1(\y \in [0,1]^n) f(\y) d\lambda}{Z(G)/N^n} \leq e^{1/n},\]
implying that
\[1 - O(1/n) \leq \frac{Z(G)/N^n}{\int 1(\y \in [0,1]^n) f(\y) d\lambda} \leq 1 + O(1/n).\]
Now, let $\tilde Z(G)$ be the estimate of $Z(G)$ produced by algorithm \ref{alg:Z} when $d = O(\log(Nn)) = O(\log(n k |E|))$. By theorem \ref{final alg}, we must have that
\[1 - O(1/n) \leq \frac{\tilde Z(G)}{Z(G)} \leq 1 + O(1/n).\]
Finally, we observe that
\[\(\frac{Z(G)/N^n}{\int 1(\y \in [0,1]^n) f(\y) d\lambda}\)\(\frac{\tilde Z(G)}{Z(G)}\) = \frac{\tilde Z(G)/N^n}{\int 1(\y \in [0,1]^n) f(\y) d\lambda},  \]
which means
\[(1-O(1/n))^2 = 1 - O(1/n) \leq \frac{\tilde Z(G)/N^n}{\int 1(\y \in [0,1]^n) f(\y) d\lambda} \leq 1 + O(1/n) = (1 + O(1/n))^2.\]
Thus, if we set our estimate of the integral $\tilde V = \tilde Z(G)/N^n$, we will have that
\[\bigg | \frac{\tilde V}{\int 1(\y \in [0,1]^n) f(\y) d\lambda} - 1 \bigg | \leq O(1/n).\]
Further, the runtime to compute this estimate will be dominated by the runtime of algorithm \ref{alg:Z}. By Theorem \ref{final alg}, this will be $(k n |E|)^{O( \eta \log( k n |E|))}$. Observing $|E| \leq \Delta n$ and taking $\eta$, $k$, and $\Delta$ to be constants, we get a runtime of $n^{O(\log n)}$.




\end{proof} 

